Stepwise Reasoning Checkpoint Analysis: A Test Time Scaling Method to Enhance LLMs' Reasoning

Mathematical reasoning through Chain-of-Thought (CoT) has emerged as a powerful capability of Large Language Models (LLMs), which can be further enhanced through Test-Time Scaling (TTS) methods like Beam Search and DVTS. However, these methods, despite improving accuracy by allocating more computational resources during inference, often suffer from path homogenization and inefficient use of intermediate results. To address these limitations, we propose Stepwise Reasoning Checkpoint Analysis (SRCA), a framework that introduces checkpoints between reasoning steps. It incorporates two key strategies: (1) Answer-Clustered Search, which groups reasoning paths by their intermediate checkpoint answers to maintain diversity while ensuring quality, and (2) Checkpoint Candidate Augmentation, which leverages all intermediate answers for final decision-making. Our approach effectively reduces path homogenization and creates a fault-tolerant mechanism by utilizing high-quality intermediate results. Experimental results show that SRCA improves reasoning accuracy compared to existing TTS methods across various mathematical datasets.

==> tables_and_algorithm/tab1_main.tex <==
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}


\begin{table*}[t]
\centering
\setlength\tabcolsep{2pt}
\begin{tabular}{llclclclc}
\hline
\multicolumn{1}{c}{}                                       & \multicolumn{8}{c}{\textbf{Datasets}}                                                                                                                      \\ \cmidrule(lr){2-9}
\multicolumn{1}{c}{\multirow{-2}{*}{\textbf{TTS Methods}}} & \multicolumn{2}{c}{\textbf{GSM8K}} & \multicolumn{2}{c}{\textbf{MATH500}} & \multicolumn{2}{c}{\textbf{AIME}} & \multicolumn{2}{c}{\textbf{OlympiadBench}} \\ \hline
% \cmidrule(lr){1-1}\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
Greedy Search (8B)                                         & \textbf{85.75}       &             & 48.60                    &           & 18.86                   &         & 15.26                       &              \\ \cdashline{1-9}
Greedy Search                                              & 43.75                &             & 24.40                    &           & 3.22                    &         & 4.59                        &              \\
 
Self-Consistency                                           & 54.36                &             & 33.00                    &           & 4.39                    &         & 9.93                        &              \\
\rowcolor[HTML]{DAE9F8} 
BoN                                                        & 72.25          & -                              & 38.60                & -                               & 6.86                 & -                               & 12.44                & -                              \\
\rowcolor[HTML]{DAE9F8} 
Weighted BoN                                               & 63.08          & {\color[HTML]{CB0000} (-9.17)} & 37.20                & {\color[HTML]{CB0000} (-1.40)}  & 6.32                 & {\color[HTML]{CB0000} (-0.54)}  & 11.70                & {\color[HTML]{CB0000} (-0.74)} \\
\rowcolor[HTML]{DAE9F8} 
Beam Search                                                & 75.05          & {\color[HTML]{CB0000} (+2.80)} & 46.60                & {\color[HTML]{CB0000} (+8.00)}  & 12.86                & {\color[HTML]{CB0000} (+6.00)}  & 12.44                & {\color[HTML]{CB0000} (0.00)}  \\
\rowcolor[HTML]{DAE9F8} 
DVTS                                                       & 74.52          & {\color[HTML]{CB0000} (+2.27)} & 46.40                & {\color[HTML]{CB0000} (+7.80)}  & 14.89                & {\color[HTML]{CB0000} (+8.03)}  & 16.74                & {\color[HTML]{CB0000} (+4.30)} \\
\rowcolor[HTML]{DAE9F8} 
SRCA                                                       & {\ul 80.67}    & {\color[HTML]{CB0000} (+8.42)} & {\ul \textbf{51.20}} & {\color[HTML]{CB0000} (+12.60)} & {\ul \textbf{21.33}} & {\color[HTML]{CB0000} (+14.47)} & {\ul \textbf{18.22}} & {\color[HTML]{CB0000} (+5.78)} \\ \hline
\end{tabular}
\caption{TODO}
\label{tab:tab1_main_res}
\end{table*}
